PriorBand: Practical Hyperparameter Optimization in the Age of Deep Learning

Hyperparameters of Deep Learning (DL) pipelines are crucial for their downstream performance. While a large number of methods for Hyperparameter Optimization (HPO) have been developed, their incurred costs are often untenable for modern DL. Consequently, manual experimentation is still the most prevalent approach to optimize hyperparameters, relying on the researcher's intuition, domain knowledge, and cheap preliminary explorations. To resolve this misalignment between HPO algorithms and DL researchers, we propose PriorBand, an HPO algorithm tailored to DL, able to utilize both expert beliefs and cheap proxy tasks. Empirically, we demonstrate PriorBand's efficiency across a range of DL benchmarks and show its gains under informative expert input and robustness against poor expert beliefs

==> captions/exp-async-bo-table-max_fidelity_loss.tex <==
Table comparing Asynchronous-HyperBand, Asynchronous-HyperBand+BO (Mobster) and Mobster+\E{} final validation errors of the current incumbent at the highest fidelity at $2$ budget horizons of $1\times$ and $5\times$. Runs are averaged over $10$ seeds where each run is with $4$ workers.

==> captions/pi-bo-table-max_fidelity_loss.tex <==
Table comparing Asynchronous-HyperBand+BO (Mobster), Asynchronous-HyperBand+\E{}+BO with models per rung (AsyncHB+PB(BO)[r]) and Asynchronous-HyperBand+\E{}+BO with a joint model (AsyncHB+PB(BO)[j]) final validation errors of the current incumbent at the highest fidelity at $2$ budget horizons of $1\times$ and $5\times$. Runs are averaged over $10$ seeds where each run is with $4$ workers.

==> tables/exp-async-bo-table-max_fidelity_loss.tex <==
\begin{table}
\caption{\protect\input{captions/exp-async-bo-table-max_fidelity_loss}}
\label{table:exp-async-bo-table-max_fidelity_loss}
\begin{center}
\scalebox{0.55}{
\centering\begin{tabular}{l | ccc | ccc}
\toprule
{} & \multicolumn{3}{c}{1x} & \multicolumn{3}{c}{5x} \\
{} &               AsyncHB &               Mobster &           Mobster(+E) &          AsyncHB &               Mobster &           Mobster(+E) \\
\midrule
\textbf{PD1-WMT (\textasciitilde  opt)     } &        $0.443\pm0.06$ &        $0.45\pm0.065$ &   $\bm{0.368\pm0.04}$ &  $0.402\pm0.027$ &       $0.374\pm0.015$ &  $\bm{0.348\pm0.023}$ \\
\textbf{PD1-Cifar100 (\textasciitilde  opt)} &       $0.434\pm0.172$ &       $0.434\pm0.172$ &  $\bm{0.259\pm0.083}$ &  $0.279\pm0.032$ &       $0.252\pm0.029$ &  $\bm{0.217\pm0.033}$ \\
\textbf{PD1-LM1B (\textasciitilde  opt)    } &       $0.663\pm0.015$ &       $0.663\pm0.012$ &  $\bm{0.639\pm0.018}$ &  $0.655\pm0.016$ &        $0.647\pm0.01$ &  $\bm{0.634\pm0.012}$ \\
\textbf{PD1-ImageNet (\textasciitilde  opt)} &       $0.333\pm0.056$ &       $0.338\pm0.056$ &   $\bm{0.261\pm0.06}$ &  $0.255\pm0.011$ &       $0.249\pm0.023$ &  $\bm{0.214\pm0.017}$ \\
\textbf{JAHS-FM (\textasciitilde  opt)     } &       $6.245\pm0.999$ &       $6.172\pm1.015$ &  $\bm{4.713\pm0.052}$ &  $5.134\pm0.274$ &       $5.177\pm0.279$ &  $\bm{4.713\pm0.052}$ \\
\textbf{JAHS-C10 (\textasciitilde  opt)    } &      $12.192\pm1.558$ &      $12.192\pm1.558$ &  $\bm{8.281\pm0.221}$ &  $9.901\pm0.598$ &       $9.872\pm0.579$ &   $\bm{8.18\pm0.177}$ \\
\textbf{JAHS-CH (\textasciitilde  opt)     } &       $6.771\pm1.296$ &       $6.771\pm1.296$ &  $\bm{4.466\pm0.188}$ &  $5.565\pm0.342$ &       $5.565\pm0.342$ &  $\bm{4.466\pm0.188}$ \\
\hline
\textbf{PD1-WMT (good)     } &        $0.45\pm0.065$ &        $0.45\pm0.065$ &    $\bm{0.372\pm0.0}$ &  $0.398\pm0.019$ &       $0.377\pm0.017$ &   $\bm{0.37\pm0.006}$ \\
\textbf{PD1-LM1B (good)    } &       $0.665\pm0.013$ &       $0.663\pm0.012$ &    $\bm{0.651\pm0.0}$ &  $0.655\pm0.013$ &       $0.649\pm0.009$ &  $\bm{0.646\pm0.008}$ \\
\textbf{JAHS-FM (good)     } &       $6.184\pm1.009$ &       $6.245\pm0.999$ &    $\bm{5.042\pm0.0}$ &  $5.126\pm0.211$ &       $5.134\pm0.274$ &   $\bm{5.013\pm0.06}$ \\
\textbf{PD1-Cifar100 (good)} &       $0.434\pm0.172$ &       $0.434\pm0.172$ &    $\bm{0.259\pm0.0}$ &  $0.279\pm0.032$ &       $0.252\pm0.029$ &  $\bm{0.226\pm0.017}$ \\
\textbf{JAHS-CH (good)     } &       $6.771\pm1.296$ &       $6.768\pm1.295$ &    $\bm{6.603\pm0.0}$ &  $5.565\pm0.342$ &       $5.668\pm0.371$ &  $\bm{5.492\pm0.312}$ \\
\textbf{JAHS-C10 (good)    } &      $12.192\pm1.558$ &      $12.192\pm1.558$ &   $\bm{10.194\pm0.0}$ &  $9.901\pm0.598$ &       $9.952\pm0.637$ &   $\bm{9.297\pm0.39}$ \\
\textbf{PD1-ImageNet (good)} &       $0.333\pm0.056$ &       $0.333\pm0.056$ &    $\bm{0.224\pm0.0}$ &  $0.254\pm0.011$ &       $0.244\pm0.013$ &  $\bm{0.222\pm0.005}$ \\
\hline
\textbf{JAHS-C10 (bad)     } &  $\bm{12.135\pm1.62}$ &      $12.375\pm1.474$ &      $13.857\pm3.841$ &  $9.869\pm0.586$ &       $9.792\pm0.624$ &  $\bm{9.744\pm0.643}$ \\
\textbf{JAHS-FM (bad)      } &  $\bm{6.184\pm1.009}$ &       $6.245\pm0.999$ &       $7.244\pm3.419$ &  $5.175\pm0.274$ &  $\bm{5.134\pm0.274}$ &       $5.181\pm0.266$ \\
\textbf{PD1-ImageNet (bad) } &       $0.335\pm0.058$ &  $\bm{0.333\pm0.056}$ &       $0.558\pm0.155$ &  $0.258\pm0.015$ &  $\bm{0.244\pm0.013}$ &       $0.248\pm0.028$ \\
\textbf{PD1-LM1B (bad)     } &       $0.665\pm0.013$ &  $\bm{0.663\pm0.012}$ &       $0.699\pm0.034$ &  $0.654\pm0.013$ &  $\bm{0.649\pm0.009}$ &       $0.657\pm0.006$ \\
\textbf{PD1-Cifar100 (bad) } &  $\bm{0.434\pm0.172}$ &       $0.434\pm0.172$ &       $0.678\pm0.195$ &  $0.279\pm0.032$ &  $\bm{0.252\pm0.029}$ &       $0.258\pm0.025$ \\
\textbf{PD1-WMT (bad)      } &   $\bm{0.45\pm0.065}$ &        $0.45\pm0.065$ &        $0.609\pm0.16$ &  $0.398\pm0.019$ &       $0.375\pm0.013$ &  $\bm{0.372\pm0.017}$ \\
\textbf{JAHS-CH (bad)      } &       $6.771\pm1.296$ &  $\bm{6.768\pm1.295}$ &       $9.218\pm2.769$ &  $5.565\pm0.342$ &       $5.668\pm0.371$ &   $\bm{5.56\pm0.707}$ \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table}

==> tables/pi-bo-table-max_fidelity_loss.tex <==
\begin{table}
\caption{\protect\input{captions/pi-bo-table-max_fidelity_loss}}
\label{table:pi-bo-table-max_fidelity_loss}
\begin{center}
\scalebox{0.55}{
\centering\begin{tabular}{l | cccc | cccc}
\toprule
{} & \multicolumn{4}{c}{5x} & \multicolumn{4}{c}{12x} \\
{} &              RS+Prior &               πBO &             PriorBand &           PriorBand+BO &               RS+Prior &                   πBO &             PriorBand &          PriorBand+BO \\
\midrule
\textbf{LC-126026 (\textasciitilde  opt)   } &       $0.026\pm0.008$ &   $0.026\pm0.008$ &  $\bm{0.024\pm0.008}$ &        $0.024\pm0.007$ &        $0.026\pm0.006$ &       $0.024\pm0.006$ &  $\bm{0.023\pm0.006}$ &       $0.024\pm0.006$ \\
\textbf{PD1-LM1B (\textasciitilde  opt)    } &       $0.648\pm0.021$ &   $0.648\pm0.021$ &  $\bm{0.637\pm0.015}$ &        $0.639\pm0.016$ &        $0.642\pm0.018$ &        $0.64\pm0.019$ &  $\bm{0.632\pm0.015}$ &       $0.637\pm0.013$ \\
\textbf{LC-189906 (\textasciitilde  opt)   } &       $0.113\pm0.013$ &   $0.113\pm0.013$ &  $\bm{0.113\pm0.015}$ &        $0.113\pm0.015$ &        $0.112\pm0.011$ &         $0.11\pm0.01$ &  $\bm{0.107\pm0.011}$ &        $0.11\pm0.012$ \\
\textbf{LC-168910 (\textasciitilde  opt)   } &  $\bm{0.199\pm0.022}$ &   $0.199\pm0.022$ &         $0.2\pm0.021$ &          $0.2\pm0.021$ &        $0.198\pm0.021$ &  $\bm{0.191\pm0.022}$ &       $0.194\pm0.019$ &         $0.2\pm0.021$ \\
\textbf{LC-168330 (\textasciitilde  opt)   } &       $0.293\pm0.037$ &   $0.293\pm0.037$ &   $\bm{0.29\pm0.041}$ &        $0.295\pm0.044$ &         $0.288\pm0.03$ &       $0.278\pm0.028$ &  $\bm{0.275\pm0.028}$ &       $0.293\pm0.043$ \\
\textbf{LC-167190 (\textasciitilde  opt)   } &       $0.139\pm0.015$ &   $0.139\pm0.015$ &  $\bm{0.136\pm0.017}$ &        $0.137\pm0.017$ &        $0.138\pm0.014$ &       $0.134\pm0.011$ &  $\bm{0.133\pm0.013}$ &       $0.135\pm0.015$ \\
\textbf{JAHS-FM (\textasciitilde  opt)     } &   $\bm{4.71\pm0.048}$ &    $4.71\pm0.048$ &        $4.724\pm0.06$ &         $4.724\pm0.06$ &         $4.71\pm0.048$ &  $\bm{4.701\pm0.046}$ &       $4.719\pm0.055$ &        $4.724\pm0.06$ \\
\textbf{JAHS-CH (\textasciitilde  opt)     } &       $4.485\pm0.114$ &   $4.485\pm0.114$ &  $\bm{4.449\pm0.124}$ &        $4.456\pm0.129$ &        $4.481\pm0.112$ &        $4.45\pm0.107$ &  $\bm{4.445\pm0.127}$ &       $4.452\pm0.127$ \\
\textbf{PD1-WMT (\textasciitilde  opt)     } &       $0.356\pm0.035$ &   $0.356\pm0.035$ &       $0.357\pm0.029$ &   $\bm{0.356\pm0.028}$ &        $0.348\pm0.025$ &  $\bm{0.345\pm0.025}$ &       $0.347\pm0.025$ &       $0.349\pm0.024$ \\
\textbf{PD1-Cifar100 (\textasciitilde  opt)} &  $\bm{0.251\pm0.044}$ &   $0.251\pm0.044$ &       $0.257\pm0.051$ &        $0.257\pm0.051$ &        $0.237\pm0.034$ &  $\bm{0.233\pm0.034}$ &        $0.238\pm0.04$ &       $0.235\pm0.033$ \\
\textbf{JAHS-C10 (\textasciitilde  opt)    } &  $\bm{8.232\pm0.229}$ &   $8.232\pm0.229$ &       $8.252\pm0.215$ &        $8.252\pm0.215$ &        $8.226\pm0.227$ &   $\bm{8.152\pm0.17}$ &       $8.236\pm0.197$ &       $8.252\pm0.215$ \\
\textbf{PD1-ImageNet (\textasciitilde  opt)} &  $\bm{0.232\pm0.031}$ &   $0.232\pm0.031$ &       $0.239\pm0.038$ &         $0.241\pm0.04$ &         $0.222\pm0.02$ &  $\bm{0.221\pm0.019}$ &       $0.228\pm0.026$ &       $0.236\pm0.034$ \\
\hline
\textbf{JAHS-CH (good)     } &  $\bm{5.936\pm0.427}$ &   $5.936\pm0.427$ &       $5.974\pm0.535$ &        $5.948\pm0.546$ &        $5.578\pm0.333$ &       $5.595\pm0.323$ &       $5.589\pm0.413$ &  $\bm{5.526\pm0.503}$ \\
\textbf{PD1-WMT (good)     } &       $0.372\pm0.003$ &   $0.372\pm0.003$ &        $0.37\pm0.008$ &    $\bm{0.37\pm0.007}$ &        $0.372\pm0.003$ &       $0.371\pm0.003$ &       $0.367\pm0.009$ &  $\bm{0.364\pm0.015}$ \\
\textbf{PD1-LM1B (good)    } &       $0.651\pm0.002$ &   $0.651\pm0.002$ &       $0.647\pm0.008$ &    $\bm{0.645\pm0.01}$ &         $0.65\pm0.003$ &       $0.649\pm0.004$ &       $0.642\pm0.009$ &   $\bm{0.64\pm0.012}$ \\
\textbf{LC-189906 (good)   } &       $0.153\pm0.012$ &   $0.153\pm0.012$ &       $0.147\pm0.013$ &   $\bm{0.144\pm0.019}$ &        $0.144\pm0.011$ &       $0.147\pm0.011$ &       $0.134\pm0.013$ &  $\bm{0.124\pm0.016}$ \\
\textbf{PD1-ImageNet (good)} &  $\bm{0.224\pm0.002}$ &   $0.224\pm0.002$ &       $0.224\pm0.001$ &        $0.224\pm0.001$ &        $0.223\pm0.005$ &        $0.22\pm0.007$ &  $\bm{0.219\pm0.008}$ &       $0.222\pm0.006$ \\
\textbf{LC-168910 (good)   } &       $0.326\pm0.017$ &   $0.326\pm0.017$ &  $\bm{0.313\pm0.019}$ &        $0.313\pm0.032$ &        $0.309\pm0.026$ &       $0.313\pm0.024$ &  $\bm{0.295\pm0.023}$ &       $0.299\pm0.033$ \\
\textbf{LC-168330 (good)   } &       $0.424\pm0.029$ &   $0.424\pm0.029$ &       $0.411\pm0.024$ &   $\bm{0.404\pm0.043}$ &         $0.397\pm0.03$ &       $0.396\pm0.033$ &       $0.387\pm0.035$ &  $\bm{0.368\pm0.052}$ \\
\textbf{PD1-Cifar100 (good)} &  $\bm{0.254\pm0.011}$ &   $0.254\pm0.011$ &       $0.258\pm0.002$ &        $0.258\pm0.002$ &        $0.249\pm0.014$ &       $0.247\pm0.015$ &       $0.248\pm0.013$ &  $\bm{0.244\pm0.016}$ \\
\textbf{LC-167190 (good)   } &       $0.216\pm0.014$ &   $0.216\pm0.014$ &  $\bm{0.198\pm0.026}$ &        $0.201\pm0.029$ &        $0.208\pm0.018$ &       $0.208\pm0.017$ &       $0.186\pm0.026$ &   $\bm{0.18\pm0.027}$ \\
\textbf{LC-126026 (good)   } &       $0.045\pm0.001$ &   $0.045\pm0.001$ &       $0.045\pm0.006$ &   $\bm{0.043\pm0.006}$ &        $0.044\pm0.003$ &       $0.043\pm0.003$ &       $0.043\pm0.007$ &  $\bm{0.038\pm0.006}$ \\
\textbf{JAHS-C10 (good)    } &  $\bm{9.758\pm0.435}$ &   $9.758\pm0.435$ &       $9.986\pm0.369$ &       $10.038\pm0.334$ &        $9.489\pm0.436$ &  $\bm{9.418\pm0.385}$ &       $9.457\pm0.415$ &       $9.859\pm0.391$ \\
\textbf{JAHS-FM (good)     } &        $5.04\pm0.011$ &    $5.04\pm0.011$ &       $5.037\pm0.021$ &    $\bm{5.02\pm0.067}$ &        $5.038\pm0.015$ &        $5.002\pm0.05$ &       $5.026\pm0.044$ &  $\bm{4.989\pm0.097}$ \\
\hline
\textbf{PD1-WMT (bad)      } &       $0.799\pm0.081$ &   $0.799\pm0.081$ &       $0.425\pm0.057$ &   $\bm{0.403\pm0.055}$ &        $0.743\pm0.096$ &       $0.705\pm0.121$ &       $0.383\pm0.021$ &  $\bm{0.371\pm0.021}$ \\
\textbf{LC-126026 (bad)    } &        $0.07\pm0.018$ &    $0.07\pm0.018$ &       $0.051\pm0.011$ &    $\bm{0.045\pm0.01}$ &        $0.057\pm0.008$ &       $0.057\pm0.007$ &        $0.045\pm0.01$ &   $\bm{0.038\pm0.01}$ \\
\textbf{PD1-ImageNet (bad) } &       $0.722\pm0.168$ &   $0.722\pm0.168$ &   $\bm{0.315\pm0.04}$ &        $0.326\pm0.042$ &        $0.605\pm0.188$ &       $0.612\pm0.193$ &         $0.28\pm0.03$ &  $\bm{0.272\pm0.027}$ \\
\textbf{LC-168910 (bad)    } &       $0.381\pm0.133$ &   $0.381\pm0.133$ &  $\bm{0.309\pm0.019}$ &        $0.319\pm0.046$ &        $0.316\pm0.044$ &       $0.309\pm0.042$ &  $\bm{0.297\pm0.016}$ &         $0.3\pm0.031$ \\
\textbf{JAHS-FM (bad)      } &       $6.282\pm2.062$ &   $6.282\pm2.062$ &       $5.962\pm0.973$ &   $\bm{5.742\pm0.492}$ &        $5.387\pm0.326$ &       $5.375\pm0.326$ &       $5.277\pm0.248$ &  $\bm{5.223\pm0.275}$ \\
\textbf{LC-189906 (bad)    } &       $0.464\pm0.163$ &   $0.464\pm0.163$ &        $0.167\pm0.03$ &   $\bm{0.148\pm0.019}$ &        $0.352\pm0.133$ &       $0.311\pm0.117$ &        $0.15\pm0.027$ &  $\bm{0.123\pm0.018}$ \\
\textbf{JAHS-C10 (bad)     } &      $12.382\pm5.288$ &  $12.382\pm5.288$ &      $11.729\pm1.795$ &  $\bm{11.228\pm1.336}$ &  $\bm{10.048\pm0.986}$ &      $10.081\pm1.141$ &      $10.075\pm0.777$ &      $10.108\pm0.813$ \\
\textbf{PD1-LM1B (bad)     } &       $0.814\pm0.061$ &   $0.814\pm0.061$ &       $0.656\pm0.014$ &   $\bm{0.651\pm0.018}$ &        $0.775\pm0.053$ &        $0.74\pm0.061$ &       $0.648\pm0.013$ &  $\bm{0.643\pm0.012}$ \\
\textbf{PD1-Cifar100 (bad) } &       $0.681\pm0.188$ &   $0.681\pm0.188$ &    $\bm{0.473\pm0.2}$ &          $0.473\pm0.2$ &        $0.564\pm0.178$ &       $0.495\pm0.226$ &       $0.297\pm0.058$ &  $\bm{0.266\pm0.035}$ \\
\textbf{JAHS-CH (bad)      } &       $8.116\pm2.843$ &   $8.116\pm2.843$ &       $6.553\pm1.284$ &   $\bm{6.318\pm1.019}$ &        $6.394\pm1.241$ &       $6.485\pm1.303$ &       $5.551\pm0.516$ &  $\bm{5.526\pm0.577}$ \\
\textbf{LC-167190 (bad)    } &       $0.258\pm0.047$ &   $0.258\pm0.047$ &  $\bm{0.196\pm0.024}$ &        $0.203\pm0.027$ &        $0.226\pm0.023$ &       $0.225\pm0.022$ &       $0.183\pm0.026$ &  $\bm{0.182\pm0.027}$ \\
\textbf{LC-168330 (bad)    } &       $0.499\pm0.073$ &   $0.499\pm0.073$ &       $0.424\pm0.035$ &   $\bm{0.419\pm0.036}$ &        $0.459\pm0.034$ &       $0.457\pm0.041$ &       $0.401\pm0.042$ &    $\bm{0.39\pm0.04}$ \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table}
